Needmining: Designing Digital Support to Elicit Needs from Social Media

Today's businesses face a high pressure to innovate in order to succeed in highly competitive markets. Successful innovations, though, typically require the identification and analysis of customer needs. While traditional, established need elicitation methods are time-proven and have demonstrated their capabilities to deliver valuable insights, they lack automation and scalability and, thus, are expensive and time-consuming. In this article, we propose an approach to automatically identify and quantify customer needs by utilizing a novel data source: Users voluntarily and publicly expose information about themselves via social media, as for instance Facebook or Twitter. These posts may contain valuable information about the needs, wants, and demands of their authors. We apply a Design Science Research (DSR) methodology to add design knowledge and artifacts for the digitalization of innovation processes, in particular to provide digital support for the elicitation of customer needs. We want to investigate whether automated, speedy, and scalable need elicitation from social media is feasible. We concentrate on Twitter as a data source and on e-mobility as an application domain. In a first design cycle we conceive, implement and evaluate a method to demonstrate the feasibility of identifying those social media posts that actually express customer needs. In a second cycle, we build on this artifact to additionally quantify the need information elicited, and prove its feasibility. Third, we integrate both developed methods into an end-user software artifact and test usability in an industrial use case. Thus, we add new methods for need elicitation to the body of knowledge, and introduce concrete tooling for innovation management in practice.

==> need-elicitation-table.tex <==
	\begin{table}
		\centering
		\rotatebox{90}{\begin{minipage}{\textheight}
		\centering
		\caption{Results of the expert survey evaluating traditional need elicitation methods. Pre-existence and involvement are evaluated based on literature}
		\label{tab:interviewresults}
		\begin{adjustbox}{width=1\textwidth}
			\scriptsize\begin{tabular}{|p{3.2cm}|p{1.6cm}|p{1.6cm}|p{1.6cm}|p{1.6cm}|p{1.6cm}|p{1.6cm}|p{1.6cm}|p{2.5cm}||p{1.6cm}|p{1.6cm}|} \toprule
				& \multicolumn{3}{c|}{Expense/Effort}   & Competencies: Required competencies of execution &  Innovation suitability: Suitability for innovative products/ services & Latent need detection: Suitability for latent needs & Represent\-ativeness: Transferability of findings to target group & Scalability: Increase of expenses with increasing number of participants & Pre-existence: Prodcut/ service must already exist & Involvement: Activity of participant \\
				
				& Preparation & Execution & Analysis &			 &       &       &       &    &   &   \\[0.7cm]
				\midrule
				1-to-1 interviews &  \diagbox[dir=SW, innerwidth=1.6cm ]{\textcolor{red}{3}}{\textcolor{blue}{0}}  &\diagbox[dir=SW, innerwidth=1.6cm]{\textcolor{red}{3}}{\textcolor{blue}{0.75}}&\diagbox[dir=SW, innerwidth=1.6cm]{\textcolor{red}{3.5}}{\textcolor{blue}{1}}&\diagbox[dir=SW, innerwidth=1.6cm]{\textcolor{red}{3}}{\textcolor{blue}{0}}&\diagbox[dir=SW, innerwidth=1.6cm]{\textcolor{red}{3}}{\textcolor{blue}{0.75}}&\diagbox[dir=SW, innerwidth=1.6cm]{\textcolor{red}{3}}{\textcolor{blue}{0.875}}&  \diagbox[dir=SW, innerwidth=1.6cm]{\textcolor{red}{3}}{\textcolor{blue}{0.375}}  & proportional & No & Active \\ \hline
				Focus groups &  \diagbox[dir=SW, innerwidth=1.6cm]{\textcolor{red}{3}}{\textcolor{blue}{0.5}} & \diagbox[dir=SW, innerwidth=1.6cm]{\textcolor{red}{3}}{\textcolor{blue}{0}}  &   \diagbox[dir=SW, innerwidth=1.6cm]{\textcolor{red}{4}}{\textcolor{blue}{1}}  &  \diagbox[dir=SW, innerwidth=1.6cm]{\textcolor{red}{3}}{\textcolor{blue}{0}}	&	\diagbox[dir=SW, innerwidth=1.6cm]{\textcolor{red}{3}}{\textcolor{blue}{0.75}} &\diagbox[dir=SW, innerwidth=1.6cm]{\textcolor{red}{2.5}}{\textcolor{blue}{0.875}}  &   \diagbox[dir=SW, innerwidth=1.6cm]{\textcolor{red}{3}}{\textcolor{blue}{0.375}}   &  below proportional  & No & Active \\ \hline
				Lead user &      \diagbox[dir=SW, innerwidth=1.6cm]{\textcolor{red}{5}}{\textcolor{blue}{0.875}} & \diagbox[dir=SW, innerwidth=1.6cm]{\textcolor{red}{5}}{\textcolor{blue}{1}}  &   \diagbox[dir=SW, innerwidth=1.6cm]{\textcolor{red}{3}}{\textcolor{blue}{1}}  &  \diagbox[dir=SW, innerwidth=1.6cm]{\textcolor{red}{4}}{\textcolor{blue}{1}}	&	\diagbox[dir=SW, innerwidth=1.6cm]{\textcolor{red}{5}}{\textcolor{blue}{0}} &\diagbox[dir=SW, innerwidth=1.6cm]{\textcolor{red}{5}}{\textcolor{blue}{0.5}}  &   \diagbox[dir=SW, innerwidth=1.6cm]{\textcolor{red}{3}}{\textcolor{blue}{0}}   & proportional & No & Active \\ \hline
				Empathic design &    \diagbox[dir=SW, innerwidth=1.6cm]{\textcolor{red}{4.5}}{\textcolor{blue}{1}} & \diagbox[dir=SW, innerwidth=1.6cm]{\textcolor{red}{5}}{\textcolor{blue}{0}}  &   \diagbox[dir=SW, innerwidth=1.6cm]{\textcolor{red}{5}}{\textcolor{blue}{0,25}}  &  \diagbox[dir=SW, innerwidth=1.6cm]{\textcolor{red}{4}}{\textcolor{blue}{1}}	&	\diagbox[dir=SW, innerwidth=1.6cm]{\textcolor{red}{5}}{\textcolor{blue}{0}} &\diagbox[dir=SW, innerwidth=1.6cm]{\textcolor{red}{5}}{\textcolor{blue}{0.25}}  &   \diagbox[dir=SW, innerwidth=1.6cm]{\textcolor{red}{3.5}}{\textcolor{blue}{0.625}}   & proportional & Yes & Passive \\ \hline
				Kansei engineering &     \diagbox[dir=SW, innerwidth=1.6cm]{\textcolor{red}{4}}{\textcolor{blue}{0.5}} & \diagbox[dir=SW, innerwidth=1.6cm]{\textcolor{red}{3.5}}{\textcolor{blue}{0.5}}  &   \diagbox[dir=SW, innerwidth=1.6cm]{\textcolor{red}{3}}{\textcolor{blue}{1.125}}  &  \diagbox[dir=SW, innerwidth=1.6cm]{\textcolor{red}{4,5}}{\textcolor{blue}{0.625}}	&	\diagbox[dir=SW, innerwidth=1.6cm]{\textcolor{red}{4}}{\textcolor{blue}{0.875}} &\diagbox[dir=SW, innerwidth=1.6cm]{\textcolor{red}{3}}{\textcolor{blue}{0.5}}  &   \diagbox[dir=SW, innerwidth=1.6cm]{\textcolor{red}{3}}{\textcolor{blue}{0}}   & below proportional & Yes & Active\\ \hline
				House of Quality &     \diagbox[dir=SW, innerwidth=1.6cm]{\textcolor{red}{3}}{\textcolor{blue}{0.75}} & \diagbox[dir=SW, innerwidth=1.6cm]{\textcolor{red}{4}}{\textcolor{blue}{1}}  &   \diagbox[dir=SW, innerwidth=1.6cm]{\textcolor{red}{2}}{\textcolor{blue}{1}}  &  \diagbox[dir=SW, innerwidth=1.6cm]{\textcolor{red}{4}}{\textcolor{blue}{2}}	&	\diagbox[dir=SW, innerwidth=1.6cm]{\textcolor{red}{2}}{\textcolor{blue}{0.875}} &\diagbox[dir=SW, innerwidth=1.6cm]{\textcolor{red}{1}}{\textcolor{blue}{0.5}}  &   \diagbox[dir=SW, innerwidth=1.6cm]{\textcolor{red}{3}}{\textcolor{blue}{1}}   & proportional & No & Passive \\ \hline
				Kano method &       \diagbox[dir=SW, innerwidth=1.6cm]{\textcolor{red}{1.5}}{\textcolor{blue}{0.875}} & \diagbox[dir=SW, innerwidth=1.6cm]{\textcolor{red}{3}}{\textcolor{blue}{0.25}}  &   \diagbox[dir=SW, innerwidth=1.6cm]{\textcolor{red}{1.5}}{\textcolor{blue}{0.625}}  &  \diagbox[dir=SW, innerwidth=1.6cm]{\textcolor{red}{2}}{\textcolor{blue}{1.125}}	&	\diagbox[dir=SW, innerwidth=1.6cm]{\textcolor{red}{3}}{\textcolor{blue}{0}} &\diagbox[dir=SW, innerwidth=1.6cm]{\textcolor{red}{2}}{\textcolor{blue}{1}}  &   \diagbox[dir=SW, innerwidth=1.6cm]{\textcolor{red}{3}}{\textcolor{blue}{0.125}}   & proportional & No & Active \\ \hline
				Persona &      \diagbox[dir=SW, innerwidth=1.6cm]{\textcolor{red}{3}}{\textcolor{blue}{0.5}} & \diagbox[dir=SW, innerwidth=1.6cm]{\textcolor{red}{4}}{\textcolor{blue}{1.5}}  &   \diagbox[dir=SW, innerwidth=1.6cm]{\textcolor{red}{3}}{\textcolor{blue}{1.5}}  &  \diagbox[dir=SW, innerwidth=1.6cm]{\textcolor{red}{4}}{\textcolor{blue}{0.5}}	&	\diagbox[dir=SW, innerwidth=1.6cm]{\textcolor{red}{5}}{\textcolor{blue}{0.875}} &\diagbox[dir=SW, innerwidth=1.6cm]{\textcolor{red}{3}}{\textcolor{blue}{0}}  &   \diagbox[dir=SW, innerwidth=1.6cm]{\textcolor{red}{3}}{\textcolor{blue}{0.5}}   & proportional & No & Passive \\ \hline
				Conjoint analysis &        \diagbox[dir=SW, innerwidth=1.6cm]{\textcolor{red}{3}}{\textcolor{blue}{0.875}} & \diagbox[dir=SW, innerwidth=1.6cm]{\textcolor{red}{2}}{\textcolor{blue}{1}}  &   \diagbox[dir=SW, innerwidth=1.6cm]{\textcolor{red}{3}}{\textcolor{blue}{0.5}}  &  \diagbox[dir=SW, innerwidth=1.6cm]{\textcolor{red}{5}}{\textcolor{blue}{0.5}}	&	\diagbox[dir=SW, innerwidth=1.6cm]{\textcolor{red}{3}}{\textcolor{blue}{0.5}} &\diagbox[dir=SW, innerwidth=1.6cm]{\textcolor{red}{2}}{\textcolor{blue}{1}}  &   \diagbox[dir=SW, innerwidth=1.6cm]{\textcolor{red}{3}}{\textcolor{blue}{0.5}}   & below proportional & No & Active \\ \hline
				Discrete choice analysis &          \diagbox[dir=SW, innerwidth=1.6cm]{\textcolor{red}{4}}{\textcolor{blue}{0.5}} & \diagbox[dir=SW, innerwidth=1.6cm]{\textcolor{red}{2}}{\textcolor{blue}{1}}  &   \diagbox[dir=SW, innerwidth=1.6cm]{\textcolor{red}{4}}{\textcolor{blue}{1}}  &  \diagbox[dir=SW, innerwidth=1.6cm]{\textcolor{red}{5}}{\textcolor{blue}{0.5}}	&	\diagbox[dir=SW, innerwidth=1.6cm]{\textcolor{red}{3}}{\textcolor{blue}{0.5}} &\diagbox[dir=SW, innerwidth=1.6cm]{\textcolor{red}{2}}{\textcolor{blue}{1}}  &   \diagbox[dir=SW, innerwidth=1.6cm]{\textcolor{red}{3}}{\textcolor{blue}{0.5}}   & below proportional & No & Active \\ \hline
	\end{tabular}	
	\end{adjustbox}	
\begin{tablenotes}
	\small
	\item Possible answers for criteria 1 to 5 : 1(low) - 2 - 3(medium) - 4 - 5(high) 
	\item \textcolor{red}{red}: median, \textcolor{blue}{blue}: semiquartile range
\end{tablenotes}	
\end{minipage}}
	\end{table}%
	

 
